Augmenting Neural Networks with First-order Logic

Today, the dominant paradigm for training neural networks involves minimizing task loss on a large dataset. Using world knowledge to inform a model, and yet retain the ability to perform end-to-end training remains an open question. In this paper, we present a novel framework for introducing declarative knowledge to neural network architectures in order to guide training and prediction. Our framework systematically compiles logical statements into computation graphs that augment a neural network without extra learnable parameters or manual redesign. We evaluate our modeling strategy on three tasks: machine comprehension, natural language inference, and text chunking. Our experiments show that knowledge-augmented networks can strongly improve over baselines, especially in low-data regimes.

==> old/base-model.tex <==
\section{Attention Model} \label{sec:model}

\tl{This section is to be removed}

Natural Language Inference~\cite{maccartney2009natural} is a task to classify the entailment relationship between a premise sentence $P$ and a hypothesis sentence $H$ that whether the textual information of $H$ is logically embedded in that of $P$.  The prediction is one of three labels $\{Entailment, Contradiction, Neutral\}$. Many neural models~\cite{parikh2016decomposable},~\cite{chen2017enhanced} have performed strongly on this task. We will focus on the Decomposable Attention model~\cite{parikh2016decomposable} and demonstrate how to build our Declarative Constrained Networks in an off-the-shelf neural networks.

The Decomposable Attention model is an end-to-end model that takes embeddings of $(P,H)$ as input and output a probability distribution over entailment labels. The pipeline can be separated into three phases: encoder, attention and classifier. Here we briefly formalize these three layers in the following subsections.

\subsection{Encoder}
The task for encoder is to generate task-specific encodings for each token given input embeddings. To distinguish them, we will use overlined symbols $\overline{\boldsymbol{P}} = (\overline{\boldsymbol{p}}_1, \overline{\boldsymbol{p}}_2, ..., \overline{\boldsymbol{p}}_m)$ to denote the input embeddings of premise sentence, and $\overline{\boldsymbol{H}} = (\overline{\boldsymbol{h}}_1, \overline{\boldsymbol{h}}_2, ..., \overline{\boldsymbol{h}}_n)$ to denote the embeddings of hypothesis. Similarly, let $\boldsymbol{P} = (\boldsymbol{p}_1, \boldsymbol{p}_2, ..., \boldsymbol{p}_m)$ and $\boldsymbol{H} = (\boldsymbol{h}_1, \boldsymbol{h}_2, ..., \boldsymbol{h}_n)$ denote the output encodings respectively. Define the encoder function as
\begin{align}
	\boldsymbol{P} &= F(\overline{\boldsymbol{P}})\\
	\boldsymbol{H} &= F(\overline{\boldsymbol{H}})
\end{align}

where $F$ function is the encoder layer. For instance $F$ could be a context-free two-layer ReLU network as in~\cite{parikh2016decomposable} or a context-dependent recurrent network as in~\cite{cheng2016long}.

\subsection{Attention} \label{sec:att}
The job of attention layer is to capture pairwise interaction between encodings from premise and hypothesis. To this end, first a pairwise similarity score is computed as
\begin{align}
	S_{ij} &= \boldsymbol{p}_i ^T \boldsymbol{h}_j
\end{align}

Let bold symbol $\boldsymbol{S}$ denote all the similarity entries as a matrix of size $m\times n$. Given $\boldsymbol{S}$, attention weights are then computed bidirectionally. That is from hypothesis to premise and from premise to hypothesis. We will use $\leftarrow$ and $\rightarrow$ to differentiate the notations. Given a premise encoding $\boldsymbol{p}_i$, a probability distribution over all $\boldsymbol{h}_j$`s are done as
\begin{align}
	\overleftarrow{\boldsymbol{a}}_i &= \frac{exp(S_{ij})}{\sum_{j \in h} exp(S_{ij})}
\end{align}

where every $\overleftarrow{\boldsymbol{a}}_i$ is of dimension $1 \times n$ naturally. Similarly, for every $\boldsymbol{h}_j$ in hypothesis, there is a probability distribution over all premise encodings:
\begin{align}
	\overrightarrow{\boldsymbol{a}}_j &= \frac{exp(S_{ij})}{\sum_{i \in p} exp(S_{ij})} \label{eq:aright}
\end{align}

where every $\overrightarrow{\boldsymbol{a}}_j$ is of $1 \times m$ dimension. In case a token is not correlated with any other tokens, the model in~\cite{parikh2016decomposable} added an extra artificial encoding to both hypothesis and premise to enable token to align with empty.

\subsection{Classifier} \label{sec:cls}
Classifier handles feature conjunction of all previous features and predict a probability distribution over the three labels $\{Entailment, Contradiction, Neutral\}$. First it aggregates features using the bidirectional attentions by
\begin{align}
	\overleftarrow{\boldsymbol{u}}_i &= G([\overleftarrow{\boldsymbol{a}}_i \cdot \boldsymbol{H} | \overline{\boldsymbol{p}}_i]) \\
	\overrightarrow{\boldsymbol{u}}_j &= G([\overrightarrow{\boldsymbol{a}}_j \cdot \boldsymbol{P} | \overline{\boldsymbol{h}}_j])
\end{align}

where G is the aggregation layer (\eg, two-layer ReLU in~\cite{parikh2016decomposable}) and $[\cdot|\cdot]$ denotes concatenation. Notice the aggregation layer jointly considers embeddings, encodings and attentions. With the aggregated premise feature $\overleftarrow{\boldsymbol{u}}_i$ and hypothesis feature $\overrightarrow{\boldsymbol{u}}_j$, the classifier does further feature conjunction to predict weight on each entailment score:
\begin{align}
	\boldsymbol{z} &= Z([\sum_i \overleftarrow{\boldsymbol{u}}_i | \sum_j \overrightarrow{\boldsymbol{u}}_j]) \label{eq:yscore}\\
	\boldsymbol{y} &= softmax(\boldsymbol{z})
\end{align}

where $Z$ is another neural layer (\eg, two-layer ReLU in~\cite{parikh2016decomposable}) that generates weights for each label, $\boldsymbol{y}$ is the probability distribution over labels. For training, $\boldsymbol{y}$ is connected to multi-class cross entropy loss function. For inference, the predicted label is $\arg\max_i y_i$


In the following sections, attention layer and classifier layer will be our focus. We will first introduce a general framework to translate declarative logic into neural form. Then we will demonstrate how to inject our neural constraints into this model.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dcn_main"
%%% End:


==> old/dcn-snli.tex <==
\section{Declarative Constrained Networks on SNLI}

Based on the translation rules in Table~\ref{tab:tab1}, we define our Declarative Constrained Networks on SNLI dataset. In this section, we will first define the logic constraints for this task, then introduce how to easily build our model on top of the Decomposable Attention networks.

\subsection{Constraining Attention and Classifier}
To relax the conflict between declarative logic and anonymous neural computations, we focus on two internal layers that carry explicit meanings. That are attention layer (as in Section~\ref{sec:att}) and classifier layer (as in Section~\ref{sec:cls}). As noted in Section~\ref{sec:model}, attention capures pairwise correlation while the prediction score $\boldsymbol{y}$ represents the weight of entailment labels. We exploit these propeties to design task-specific neural constraints using the translation rules in Table~\ref{tab:tab1}.

For ease of notation, we will let $i$ to denote a token or its Part-of-Speech tag from the premise sentence, and $j$ to denote a token or corresponding Part-of-Speech tag from the hypothesis. Also notice there are two versions of attention in Section~\ref{sec:att}. We concentrate on $\overrightarrow{\boldsymbol{a}}$ because we care more about the mapping from hypothesis to premise. In the following subsections, let $\overrightarrow{a}_{ij}$ to indicate alignment between $(i,j)$, let $\{Ent,Con,Neu\}$ denote the set of prediction labels (which implicitly maps to $\boldsymbol{y})$.

We separate the constraints into two categories according to different application senarios. One is within-layer constraints that imposes structure information into the attention layer regardless of states of the classifier. Another is cross-layer constraints that bridge structural interaction between attention and classifier layers.

\subsubsection{Within-layer Constraints} \label{sec:within}
We introduce three simple within-layer constraints on the attention phase in Table~\ref{tab:tab2}.

To explain, the purpose of Constraint w1 is to prohibit punctuation from aligning to non-punctuation token. Constraint w2 means to limit the alignment between determiners and numbers. The last constraint recommends the alignment if the pair is either synonym or antonym.

\begin{table}[t]
\begin{center}
\begin{tabular}{|l|l|}
\hline \bf Id. & \bf Logic Constraint \\ \hline
w1 & $\displaystyle \big( Punct(i) \wedge \neg Punct(j) \big) \vee$ \\
	& \hspace{2ex} $\displaystyle \big( \neg Punct(i) \wedge Punct(j) \big) \rightarrow \neg \overrightarrow{a}_{ij}$\\
w2 & $\displaystyle \big( Det(i) \vee Num(i) \big) \wedge $ \\
	& \hspace{2ex} $\displaystyle \big( Det(j) \vee Num(j) \vee Nul(j) \big) \rightarrow \overrightarrow{a}_{ij}$ \\
w3 & $\displaystyle Syn(i,j) \vee Ant(i,j) \rightarrow \overrightarrow{a}_{ij}$ \\
\hline
\end{tabular}
\end{center}
\caption{Within-layer Constraints. $Punct$, $Det$, $Num$ are Part-of-Speech tag indicators. $Syn$ and $Ant$ are synonym and anotnym indicators. $Nul$ indicates whether a token is the artificial token noted in Section~\ref{sec:att}}
\label{tab:tab2}
\end{table}

\subsubsection{Cross-layer Constraints}
To model the structural interaction between attention and classification layer, we introduce two cross-layer constraints in Table~\ref{tab:tab3}.

\begin{table}[t]
\begin{center}
\begin{tabular}{|l|l|}
\hline \bf Id. & \bf Logic Constraint \\ \hline
c1 & $\displaystyle \bigvee_{i\in Oppo(i,j)} \overrightarrow{a}_{ij} \leftrightarrow b_{j}$\\
	& \hspace{2.5ex} $\displaystyle \bigvee_j b_j \rightarrow \neg Ent$\\
c2 & $\displaystyle \bigvee_{i\in P} \overrightarrow{a}_{ij} \leftrightarrow b_{j}$ \\
	& \hspace{2.5ex} $\displaystyle \bigvee_j \neg b_j \rightarrow Neu$\\
\hline
\end{tabular}
\end{center}
\caption{Cross-layer Constraints. }
\label{tab:tab3}
\end{table}

Cross-layer constraint c1 promote labels except $Ent$ if there is an alignment with opposite meaning which is denoted as relation $Oppo(i,j)$. Note the relation $Oppo$ could be different from $Ant$ (as in Subsection~\ref{sec:within}). On the other hand, constraint c2 says that if there is no hypothesis token aligned to premise token significantly, the prediction label should be $Neu$.


\subsection{Plug and Play}
We demonstrate how to build our Declarative Constrained Model by connecting neural constraints to the computation graph of an existing neural model. For within-layer constraints, we redefine the pairwise score $\boldsymbol{S}$ (in Section~\ref{sec:att}) and the attention $\overrightarrow{\boldsymbol{a}}$ as
\begin{align}
	\boldsymbol{S}^\prime &= \sum_{w\in \{w1,w2,w3\}} -\rho \cdot \boldsymbol{d}(w, \overrightarrow{\boldsymbol{a}}) + \boldsymbol{S} \\
	\overrightarrow{\boldsymbol{a}}^\prime_j &= \frac{exp(S^\prime_{ij})}{\sum_{i \in p} exp(S^\prime_{ij})}
\end{align}

where $\boldsymbol{d}(w, \overrightarrow{\boldsymbol{a}})$ is the distance function for within-layer constraint $w$. Similarly, we can redefine the prediction score $\boldsymbol{y}$ to incorporate cross-layer constraints:
\begin{align}
	\boldsymbol{y}^\prime &= \sum_{c\in \{c1,c2\}} -\rho \cdot \boldsymbol{d}(c, \boldsymbol{y}) + \boldsymbol{y}
\end{align}

where $\boldsymbol{d}(c, \boldsymbol{y})$ are the distances of prediction labels given cross-layer constraint $c$.

By replace $\boldsymbol{S}$, $\overrightarrow{\boldsymbol{a}}$ and $\boldsymbol{y}$ with redefined versions, we have a fully differentiable constrained neural networks ready for training. In the next section, we show that by using neural constraints, our model is able to learn better than unconstrained model from small amount of data.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dcn_main"
%%% End:


==> old/problem.tex <==
\section{Neural Networks \& Constraints}
\label{sec:neural-networks-constraints}

%Neural networks are expressive enough to capture any functional
%input-output
%relationships~\cite[\eg][]{cybenko1989approximation}. However,
%expressiveness does not guarantee learnability. In practice,
%learning neural models has proven to be difficult for several
%reasons.  First, the non-convexity of loss functions means that
%learning is sensitive both to parameter initialization~\cite{glorot2010understanding}
%and design choices such as the learning rate decay method.
%Second, modern neural architectures demand massive data to
%train their large number of learnable parameters.
%
%Crucially, neural models for a task are typically trained
%end-to-end. Feedback at the output level is used to supervise all
%the trainable parameters. While end-to-end learning is undeniably
%successful, often, we may have access to knowledge about a problem
%that is easy to state in a declarative fashion. Such declarative
%knowledge could be of linguistic (\eg, \example{adjectives can not
%  modify nouns}) or pragmatic (\eg, \example{an event can not both
%  the cause and effect of another}) in origin. Should neural
%networks have to learn such easily stated knowledge from data?  We
%need a mechanism for systematically introducing such knowledge into
%both the training and prediction phases.

% Neural networks offer the ability to easily define fully
% differentiable expressive classifiers that can be trained by
% backpropagation using efficient software infrastructure.

Neural models are typically trained in end-to-end fashion where 
 feedback at the output level is used to supervise all the trainable parameters.
While such setup is undeniably successful, often, we may have access to knowledge
 about a problem that is easy to state in delcarative rules.
Such knowledge could be of linguistic form (\eg, \example{adjectives can not
 modify nouns}) or pragmatic form (\eg, \example{an event can not both
 the cause and effect of another}). 
How can neural networks learn to use these kind of easily stated knowledge?
We need a mechanism for systematically introducing it into both the training and prediction phase.

In this paper, we present {\em Declaratively Constrained Attention Networks
 (\theModels)}, a modeling framework that uses declarative knowledge
 to constrain neurons.
Using our framework, model designers can write declarative constraints in first order logic which are
 compiled into differentiable computation graph.
The process only augment the architecture of an existing neural network, but introduce no more parameter to learn.


% key idea: naming neurons -- usually in the standard end-to-end
% approach, the input and the output neurons have meaning. this is
% already a starting point. sometimes, maybe even the inner ones
% have meaning.
%
The ability to incorporate logic into a neural network hinges on
 the groundings of neurons.
Typically, only the output neurons of an end-to-end neural networks 
 have well defined meanings.
For instance, they are dictated by multiclass classification task.
In attention models, attention neuron is designed to represent word alignment or word selection.
We will focus on these two types of neurons.
However note that, to apply our framework, not every neuron needs to have grounding.
For the easy of illustration, we will assume that named neurons all have well-defined meanings,
unless explicitly noted.


%an end-to-end
%trained network, only the input and output nodes of the network have
%externally defined meaning; these are dictated by the task being
%solved. For example, for the NLI task, input neurons correspond to
%words in the premise and the hypothesis, and the outputs correspond
%to the three decisions (entail, contradict and neutral) that the
%network can make. The inner nodes in the network are usually
%anonymous units of differentiable compute.  But there are indeed
%certain inner nodes that also carry explicit meanings. For example,
%the attention nodes have the implied interpretation
%of alignments between premise-hypothesis words.

%Naming a node in the computation graph (\eg, attention, entail,
%etc.) gives us the opportunity to reason about and ascribe external
%meaning to it. (Indeed, we could argue that network designers have
%intended meaning in mind when the node is named.) Note that not every
%neuron need to be named. Some nodes may exist purely to transform feature representations.

A typical neural layer could be computed as $\ba = g\p{\bW \bx}$ where 
 $g$ is an activation function that outputs $[0,1]$, $\bW$ are learnable weights,
 $\ba$ are grounded output neurons,
 and $\bx$ are the immediate input features that do not necessarily have grounding.

In the computational graph, assume $\ba$ are downstream neurons and $\bb$ are neurons
 from a upstream layer.
To capture the mutual constraint between $\ba$ and $\bb$,
 we generalize the definition of the layer as
\begin{align}
	\ba &= g \p{\bW \bx + \rho d_c\p{\bb}}	\label{eq:topfunc}
\end{align}

Here, $d_c$ represents a {\em constraint distance function} that describes how much the corresponding
 values of $\ba$ should be to satisfy the constraint $c$ given values of $\bb$.
The relative impact of constraint $c$ is controlled by the scaling factor $\rho$.

% where $\rho$ is a scaling scalar variable; $d(\boldsymbol{b})$
% represents a set of assigned features. Considering that
% $\boldsymbol{W}$ is a matrix and $\phi(\boldsymbol{b})$ is a column
% vector, the output dimension of $d(\boldsymbol{b})$ must be the same
% as $\boldsymbol{a}$. 

The $d$ function can be thought of as a way to encode information from external knowledge.
For instance, in the previous example, we can think of $\ba$ is the entailment prediction
 while $\bb$ represents word alignments.
We can thus define constraint $c$ as \emph{any unaligned word in the hypothesis $\rightarrow$ non-entailment}.
As noted previously, with attention models, it is easy to find neurons with groundings that correspond to predicates in the constraint.
However, the indifferentiability of logical statement is incompatible with differentiable neural networks.
Therefore, in the following sections, we will show how to compile logical statement into computational graph,
 i.e. the $d$ function;
and how to use the compiled graph to augment the existing graph of neural networks.

\paragraph{Comment} It is important to distinguish named neuron from the predicates in constraint.
We will use lower case for neuron while upper case for predicates, unless otherwise noted.
%For instance, we define $B_i$ the predicate \emph{word $i$ is unaligned in the hypothesis} corresponding to neurons $\bb$,
% and $A$ the predicate \emph{non-entailment} corresponding to neuron $\ba$.




% what do we get by naming neurons: a simple example

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dcn_main"
%%% End:

